Energy norm analysis of exactly symmetric mixed finite elements for linear elasticity

We consider mixed finite element methods with exact symmetric stress tensors. We derive a new quasi-optimal a priori error estimate uniformly valid with respect to the compressibility. For the a posteriori error analysis we consider the Prager-Synge hypercircle principle and introduce a new estimate uniformly valid in the incompressible limit. All estimates are validated by numerical examples.

==> conv_data/0.25_circ_JM.tex <==
202&\numnum{0.04287133477774831}&--&\numnum{0.1115488187843652}&--&\numnum{0.042824468524620685}&--&\numnum{0.11595673286143118}&--&\numnum{0.06181144608779752}&--&\num{0.9381545591676098}\\
808&\numnum{0.018033346017609368}&\numeoc{1.2493462273561877}&\numnum{0.04610220519340681}&\numeoc{1.274767571208236}&\numnum{0.018011684260197936}&\numeoc{1.2495022488033387}&\numnum{0.04820615191403502}&\numeoc{1.2662974150179662}&\numnum{0.02574039082314231}&\numeoc{1.2638400589555372}&\num{0.9371046882095332}\\
3232&\numnum{0.004474325485890659}&\numeoc{2.010924993565475}&\numnum{0.012008116351305173}&\numeoc{1.9408258993466685}&\numnum{0.004468385483892885}&\numeoc{2.011107536570409}&\numnum{0.012633898780995027}&\numeoc{1.9319173513666943}&\numnum{0.006702693105223034}&\numeoc{1.941221174444238}&\num{0.9430926101622569}\\
12928&\numnum{0.00108367098808955}&\numeoc{2.0457434009702666}&\numnum{0.00329424809474276}&\numeoc{1.8659887451856565}&\numnum{0.0010821574219685905}&\numeoc{2.0458432673060885}&\numnum{0.00346732314357478}&\numeoc{1.865405716393524}&\numnum{0.0018166275491321607}&\numeoc{1.8834782151110079}&\num{0.9548468643431754}\\


==> conv_data/0.4999_circ_JM.tex <==
202&\num{0.042873156942947833}&--&\num{0.09239431426102616}&--&\num{0.04273327455625439}&--&\num{3.7042349886016344}&--&\num{1.8522407455187206}&--&\numnum{0.9999334680731221}\\
808&\num{0.018033579080053833}&\numeoc{1.2493888998552194}&\num{0.03916284265093882}&\numeoc{1.2383185868027924}&\num{0.017968925055272044}&\numeoc{1.2498557658741183}&\num{1.5875540136033988}&\numeoc{1.2223699451698267}&\num{0.7938281064220736}&\numeoc{1.2223730768071428}&\numnum{0.9999362722265145}\\
3232&\num{0.004474325512097603}&\numeoc{2.0109436303440114}&\num{0.010418795532112566}&\numeoc{1.910296983275027}&\num{0.00445659409520834}&\numeoc{2.0114906339441627}&\num{0.438003535198455}&\numeoc{1.857791258548653}&\num{0.21901315223552617}&\numeoc{1.8578091340339553}&\numnum{0.999948463200139}\\
12928&\num{0.0010836709863419342}&\numeoc{2.045743411747003}&\num{0.002924621213567254}&\numeoc{1.832866814847297}&\num{0.0010791525512830662}&\numeoc{2.0460427451929375}&\num{0.12406751733743017}&\numeoc{1.8198170675323548}&\num{0.06203611486347923}&\numeoc{1.819837266894801}&\numnum{0.9999623282434728}\\


==> conv_data/0.499_circ_JM.tex <==
202&\num{0.042873147985835414}&--&\num{0.09249699998392791}&--&\num{0.04273376473570848}&--&\num{1.1735739131113585}&--&\num{0.5871758790937764}&--&\numnum{0.99933774585051}\\
808&\num{0.018033577602689272}&\numeoc{1.2493887166354583}&\num{0.03920051939289999}&\numeoc{1.238533804848227}&\num{0.017969154283234444}&\numeoc{1.2498539102498372}&\num{0.5028894841037402}&\numeoc{1.2225954166869863}&\num{0.25160601523916354}&\numeoc{1.2226262904916014}&\numnum{0.9993654337679387}\\
3232&\num{0.004474325511920012}&\numeoc{2.0109435122113903}&\num{0.010427448302772388}&\numeoc{1.9104866100138167}&\num{0.0044566573780056625}&\numeoc{2.011488552305195}&\num{0.13869658329753087}&\numeoc{1.8583091373891305}&\num{0.0693842373022081}&\numeoc{1.8584865597241018}&\numnum{0.9994863727708979}\\
12928&\num{0.0010836709863517968}&\numeoc{2.0457434116766104}&\num{0.0029266358678692738}&\numeoc{1.8330709977872677}&\num{0.0010791686791341937}&\numeoc{2.046041670241215}&\num{0.03927839983599359}&\numeoc{1.8201241862585449}&\num{0.019646641395073272}&\numeoc{1.8203252448483866}&\numnum{0.9996243248390466}\\


==> conv_data/circ_AG_conv_data.tex <==
202&\num{0.08116566021161238}&--&\num{1.1575237789918948}&--&\num{0.15983204928075714}&--&\num{0.04297820491236226}&--\\
808&\num{0.022183777994370088}&\numeoc{1.8713643934548627}&\num{0.692092415073983}&\numeoc{0.742005232198577}&\num{0.047933130586074554}&\numeoc{1.7374616515344061}&\num{0.022846922598345337}&\numeoc{0.9116053740863824}\\
3232&\num{0.0027583613955988844}&\numeoc{3.0076216900122557}&\num{0.34846065942319754}&\numeoc{0.9899689061068181}&\num{0.006248923139268831}&\numeoc{2.939343667245014}&\num{0.003022285631177639}&\numeoc{2.9182879335623704}\\
12928&\num{0.00032946400939812585}&\numeoc{3.065618709420217}&\num{0.1746822556408554}&\numeoc{0.996262722017128}&\num{0.0007684032772213545}&\numeoc{3.023672018107542}&\num{0.0003806829051506101}&\numeoc{2.9889783224777666}\\


==> conv_data/circ_AG_conv_data_old.tex <==
204&\num{0.08205231777803892}&--&\num{1.1435694520962718}&--&\num{0.23148104830040284}&--&\num{1.1484794653208625}&--\\
816&\num{0.02215603367017931}&\numeoc{1.8888444508773226}&\num{0.6893546173503866}&\numeoc{0.7302257579874797}&\num{0.09339273926539964}&\numeoc{1.309511784342302}&\num{0.6889767676555556}&\numeoc{0.7371978206416281}\\
3264&\num{0.002817032017170876}&\numeoc{2.9754517700884824}&\num{0.3480256870748414}&\numeoc{0.9860525317021425}&\num{0.029187234696691673}&\numeoc{1.6779728620531669}&\num{0.34753981311960946}&\numeoc{0.9872770778485283}\\
13056&\num{0.00033598190599022274}&\numeoc{3.0677205157183063}&\num{0.17471159285464247}&\numeoc{0.9942184520572175}&\num{0.009703807814607257}&\numeoc{1.5887146481529557}&\num{0.1745586439307826}&\numeoc{0.9934664589688931}\\


==> conv_data/circ_JM_conv_data.tex <==
202&\num{0.35212331824017506}&--&\num{1.5458719583140863}&--&\num{1.2312599740896344}&--&\num{1.1084245363948484}&--\\
808&\num{0.1480469984663723}&\numeoc{1.2500255268956413}&\num{0.6615174074685227}&\numeoc{1.2245698026301703}&\num{0.34008450209674934}&\numeoc{1.8561702435095562}&\num{0.24022827852318307}&\numeoc{2.206032658877588}\\
3232&\num{0.03672770001096221}&\numeoc{2.0111147828310485}&\num{0.3145565184324921}&\numeoc{1.072459861859738}&\num{0.07757222263519647}&\numeoc{2.1322812187439717}&\num{0.03640077778896768}&\numeoc{2.7223648057273566}\\
12928&\num{0.008895294957991257}&\numeoc{2.0457542038429506}&\num{0.1574179826629861}&\numeoc{0.9987189021657848}&\num{0.0216256940155692}&\numeoc{1.8427937062881512}&\num{0.00855813692283617}&\numeoc{2.0886006112157056}\\


==> conv_data/circ_JM_conv_data_old.tex <==
204&\num{0.34966003274524565}&--&\num{1.3118439053819622}&--&\num{0.9378631240940861}&--&\num{0.7644014122142884}&--\\
816&\num{0.1479417523618574}&\numeoc{1.2409236311817877}&\num{0.6333858188129695}&\numeoc{1.0504395941114342}&\num{0.28685786229467264}&\numeoc{1.7090413243956157}&\num{0.16069569445273418}&\numeoc{2.249999168508734}\\
3264&\num{0.03672025935631982}&\numeoc{2.0103811159424985}&\num{0.31372793489506723}&\numeoc{1.013570571476455}&\num{0.0768371287915314}&\numeoc{1.9004605451205612}&\num{0.035928722211863794}&\numeoc{2.161121742562171}\\
13056&\num{0.008886480121435825}&\numeoc{2.0468922536567824}&\num{0.1570805745268076}&\numeoc{0.9980092152154549}&\num{0.021382615137770785}&\numeoc{1.8453653017417766}&\num{0.00837850744340185}&\numeoc{2.100372458847598}\\


==> conv_data/poly_AG_conv_data.tex <==
24&\num{0.00037605327799784913}&--&\num{0.004749853190822032}&--&\num{0.0006159226932881574}&--&\num{0.0007458918818328183}&--&\num{0.00014525523570667407}&--\\
96&\num{7.925613531084864e-05}&\numeoc{2.246342547284669}&\num{0.0028097067801935325}&\numeoc{0.7574633438370721}&\num{0.00011504215892918279}&\numeoc{2.4205866289861473}&\num{0.0001922297372183589}&\numeoc{1.9561349919059807}&\num{2.819211912523909e-05}&\numeoc{2.3652263357523404}\\
384&\num{1.1250848902249353e-05}&\numeoc{2.8164887601129793}&\num{0.0014968745136531927}&\numeoc{0.9084662971545105}&\num{1.7213724269036404e-05}&\numeoc{2.7405314853404943}&\num{2.946586706952422e-05}&\numeoc{2.7057149078703526}&\num{4.347080641202459e-06}&\numeoc{2.6971731615451575}\\
1536&\num{1.446869089053655e-06}&\numeoc{2.9590275605818914}&\num{0.0007577157835226822}&\numeoc{0.9822245768742588}&\num{2.242295922563593e-06}&\numeoc{2.9405106722666834}&\num{3.914067100522149e-06}&\numeoc{2.912304325871292}&\num{5.771914041337367e-07}&\numeoc{2.912925139147607}\\
6144&\num{1.8292106738196642e-07}&\numeoc{2.983641246674617}&\num{0.00037999419533757623}&\numeoc{0.9956794195140444}&\num{2.84607732060808e-07}&\numeoc{2.97792992570204}&\num{5.023648723835455e-07}&\numeoc{2.961860995784992}&\num{7.447619564993116e-08}&\numeoc{2.9541985295694695}\\


==> conv_data/poly_JM_conv_data.tex <==
24&\num{0.0019558123288080966}&--&\num{0.004905066493631567}&--&\num{0.00291633779069924}&--&\num{0.0030098814418773366}&--&\num{0.0016991828248104086}&--\\
96&\num{0.0007035746765729797}&\numeoc{1.4749924796050409}&\num{0.00278324410630389}&\numeoc{0.8175052471513905}&\num{0.0013947857762593163}&\numeoc{1.0641142754096937}&\num{0.0016150512161635145}&\numeoc{0.8981267447917873}&\num{0.0009919263304478346}&\numeoc{0.7765362067644381}\\
384&\num{0.00018222192304000735}&\numeoc{1.9490070179189496}&\num{0.0013948178664781193}&\numeoc{0.9966906976702332}&\num{0.0003792043971193557}&\numeoc{1.878995958568166}&\num{0.00043171806565525065}&\numeoc{1.9034185459568487}&\num{0.0002664883424203416}&\numeoc{1.8961605534023975}\\
1536&\num{4.75841439261092e-05}&\numeoc{1.9371437183005498}&\num{0.0006950828171842517}&\numeoc{1.0048199628001822}&\num{0.00010151707045633639}&\numeoc{1.9012533512020362}&\num{0.00011300857831967864}&\numeoc{1.9336571753000387}&\num{7.117814190311907e-05}&\numeoc{1.9045662463447408}\\
6144&\num{1.2205597073164184e-05}&\numeoc{1.9629380456055017}&\num{0.0003470411505042999}&\numeoc{1.002078140252189}&\num{2.6367375873451406e-05}&\numeoc{1.9448964381397267}&\num{2.8912984600178065e-05}&\numeoc{1.9666428430443996}&\num{1.843939845403328e-05}&\numeoc{1.9486426802652954}\\

